Multi-Object Discovery by Low-Dimensional Object Motion

Recent work in unsupervised multi-object segmentation shows impressive results by predicting motion from a single image despite the inherent ambiguity in predicting motion without the next image. On the other hand, the set of possible motions for an image can be constrained to a low-dimensional space by considering the scene structure and moving objects in it. We propose to model pixel-wise geometry and object motion to remove ambiguity in reconstructing flow from a single image. Specifically, we divide the image into coherently moving regions and use depth to construct flow bases that best explain the observed flow in each region. We achieve state-of-the-art results in unsupervised multi-object segmentation on synthetic and real-world datasets by modeling the scene structure and object motion. Our evaluation of the predicted depth maps shows reliable performance in monocular depth estimation.

==> figs/davis17clustering.tex <==
\begin{figure*}[t]
    \centering
     \rotatebox[origin=l]{90}{
 \parbox{0.07\linewidth}{\centering RGB}}
 % \hspace{0.001\linewidth} 
 \includegraphics[width=0.155\linewidth]{gfx/davis17/bike-packing/resize-00040.jpg}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/judo/00028.jpg}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/gold-fish/00029.jpg}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/lab-coat/00002.jpg}
    % \hspace{0.002\linewidth}
    % \includegraphics[width=0.155\linewidth]{gfx/davis17/dance-twirl/00067.jpg}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/blackswan/00002.jpg}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/mbike-trick/00078.jpg}
    
    
    \rotatebox[origin=l]{90}{
 \parbox{0.07\linewidth}{\centering Flow}}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/bike-packing/resize-00040.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/judo/00028.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/gold-fish/00029.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/lab-coat/00002.png}
    % \hspace{0.002\linewidth}
    % \includegraphics[width=0.155\linewidth]{gfx/davis17/dance-twirl/00067.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/blackswan/00002.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/mbike-trick/00078.png}


    \rotatebox[origin=l]{90}{
 \parbox{0.07\linewidth}{\centering GT}}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/bike-packing/resize-00040-gt.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/judo/00028-gt.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/gold-fish/00029-7-gt.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/lab-coat/00002-gt.png}
    % \hspace{0.002\linewidth}
    % \includegraphics[width=0.155\linewidth]{gfx/davis17/dance-twirl/00067-gt.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/blackswan/00002-gt.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/mbike-trick/00078-gt.png}


    \rotatebox[origin=l]{90}{
 \parbox{0.07\linewidth}{\centering OCLR}}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/bike-packing/resize-00040-oclr.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/judo/00028-oclr.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/gold-fish/00029-7-oclr.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/lab-coat/00002-oclr.png}
    % \hspace{0.002\linewidth}
    % \includegraphics[width=0.155\linewidth]{gfx/davis17/dance-twirl/00067-oclr.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/blackswan/00002-oclr.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/mbike-trick/00078-oclr.png}


    \rotatebox[origin=l]{90}{
 \parbox{0.07\linewidth}{\centering Ours}}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/bike-packing/resize-00040-our.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/judo/00028-our.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/gold-fish/00029-7-our.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/lab-coat/00002-our.png}
    % \hspace{0.002\linewidth}
    % \includegraphics[width=0.155\linewidth]{gfx/davis17/dance-twirl/00067-our.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/blackswan/00002-our.png}
    % \hspace{0.002\linewidth}
    \includegraphics[width=0.155\linewidth]{gfx/davis17/mbike-trick/00078-our.png}
    \caption{\textbf{Qualitative Comparison on DAVIS-2017}. 
    While OCLR~\cite{Xie2022NeurIPS} misses some objects completely and suffers from relying on only optical flow as input, our method can segment a wide variety of multiple objects on everyday scenes.}
    \label{fig:davis17clustering}
    % \vspace{-3.5pt}
\end{figure*}

==> figs/notimportant.tex <==
\begin{tabular}{lllllll}
RGB & \includegraphics[width=0.3\linewidth]{gfx/davis17/bike-packing/00040.jpg}
    &
    \includegraphics[width=0.3\linewidth]{gfx/davis17/gold-fish/00029.jpg}
    &
    \includegraphics[width=0.3\linewidth]{gfx/davis17/judo/00028.jpg}
    &
    \includegraphics[width=0.3\linewidth]{gfx/davis17/lab-coat/00002.jpg}
    &
    \includegraphics[width=0.3\linewidth]{gfx/davis17/blackswan/00002.jpg}
    &
    \includegraphics[width=0.3\linewidth]{gfx/davis17/mbike-trick/00078.jpg} \\
\end{tabular}
 

==> tab/clevr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}lcccc@{}}
\toprule
      & \multicolumn{2}{c}{CLEVR}      & \multicolumn{2}{c}{CLEVRTEX}    \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & \textbf{FG-ARI}$\uparrow$ & \textbf{mIoU}$\uparrow$ & \textbf{FG-ARI}$\uparrow$ & \textbf{mIoU}$\uparrow$ \\ \midrule
SPAIR & 77.13 & \underline{65.95} & 0.00 & 0.00    \\
% SPAIR$^\dag$ & 77.05 & 66.87 & 0.00 & 0.00    \\
MN    & 72.12 & 56.81 & 38.31 & 10.46   \\
% MN$^\dag$    & 72.08 & 57.61 & 38.34 & 10.34   \\
MONet & 54.47 & 30.66 & 36.66 & 19.78   \\
% MONet$^\dag$ & 61.36 & 45.61 & 35.64 & 23.59   \\
SA    & \textbf{95.89} & 36.61 & 62.40 & 22.58   \\
% SA$^\dag$    & 94.88 & 37.68 & 61.60 & 21.96   \\
IODINE & 93.81 & 45.14 & 59.52 & 29.17   \\
% IODINE$^\dag$ & 93.68 & 44.20 & 60.63 & 29.40   \\
DTI-S & 59.54 & 48.74 & 79.90 & 33.79   \\
% DTI-S$^\dag$ & 89.86 & 53.38 & 79.86 & 32.20   \\
GNM   & 65.05 & 59.92 & 53.37 & 42.25   \\
% GNM$^\dag$   & 65.67 & 63.38 & 53.38 & 44.30   \\
SAVi  & -    & -  & 49.54 & 31.88   \\
PPMP   & 91.69 & \textbf{66.70} & \underline{90.80} & \underline{55.07}   \\
% PMP$^\dag$   & 95.94 & 84.86 & 92.61 & \textbf{77.67}   \\
Ours  & \underline{95.03} & 63.36 & \textbf{94.66} & \textbf{64.08}   \\
% Ours$^\dag$  & \textbf{96.95} & \textbf{86.38} & \textbf{95.32} & 70.28    \\
\bottomrule    
\end{tabular}
\caption{\textbf{Multi-Object Segmentation results.} The results here \\are without any post-processing. }
\label{tab:clevr-nopp}
\end{table}

==> tab/clevr_comb.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[b]
\begin{tabular}{@{}lcccc@{}}
\toprule
      & \multicolumn{2}{c}{CLEVR}      & \multicolumn{2}{c}{CLEVRTEX}    \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & \textbf{FG-ARI}$\uparrow$ & \textbf{mIoU}$\uparrow$ & \textbf{FG-ARI}$\uparrow$ & \textbf{mIoU}$\uparrow$ \\ \midrule
SPAIR & 77.13 & \underline{65.95} & 0.00 & 0.00    \\
MN    & 72.12 & 56.81 & 38.31 & 10.46   \\
MONet & 54.47 & 30.66 & 36.66 & 19.78   \\
SA    & \textbf{95.89} & 36.61 & 62.40 & 22.58   \\
IODINE & 93.81 & 45.14 & 59.52 & 29.17   \\
DTI-S & 59.54 & 48.74 & 79.90 & 33.79   \\
GNM   & 65.05 & 59.92 & 53.37 & 42.25   \\
SAVi  & -    & -  & 49.54 & 31.88   \\
PPMP   & 91.69 & \textbf{66.70} & \underline{90.80} & \underline{55.07}   \\
Ours  & \underline{95.03} & 63.36 & \textbf{94.66} & \textbf{64.08}   \\
\bottomrule    
\end{tabular}
%
\hfill
%
\begin{tabular}{@{}lcccc@{}}
\toprule
      & \multicolumn{2}{c}{CLEVR}      & \multicolumn{2}{c}{CLEVRTEX}    \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & \textbf{FG-ARI}$\uparrow$ & \textbf{mIoU}$\uparrow$ & \textbf{FG-ARI}$\uparrow$ & \textbf{mIoU}$\uparrow$ \\ \midrule
SPAIR & 77.05 & 66.87 & 0.00 & 0.00    \\
MN    & 72.08 & 57.61 & 38.34 & 10.34   \\
MONet & 61.36 & 45.61 & 35.64 & 23.59   \\
SA    & 94.88 & 37.68 & 61.60 & 21.96   \\
IODINE & 93.68 & 44.20 & 60.63 & 29.40   \\
DTI-S & 89.86 & 53.38 & 79.86 & 32.20   \\
GNM   & 65.67 & 63.38 & 53.38 & 44.30   \\
%SAVi  & -    & -  & 49.54 & 31.88   \\
PPMP   & \underline{95.94} & \underline{84.86} & \underline{92.61} & \textbf{77.67}   \\
Ours  & \textbf{96.95} & \textbf{86.38} & \textbf{95.32} & \underline{70.28}    \\ \bottomrule    
\end{tabular}
\caption{hello}
\label{tab:clevr}
\end{table*}

==> tab/clevr_pp.tex <==
\begin{table}[]
\begin{tabular}{@{}lcccc@{}}
\toprule
      & \multicolumn{2}{c}{CLEVR}      & \multicolumn{2}{c}{CLEVRTEX}    \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & \textbf{FG-ARI}$\uparrow$ & \textbf{mIoU}$\uparrow$ & \textbf{FG-ARI}$\uparrow$ & \textbf{mIoU}$\uparrow$ \\ \midrule
% SPAIR & 77.13 & 65.95 & 0.00 & 0.00    \\
SPAIR$^\dag$ & 77.05 & 66.87 & 0.00 & 0.00    \\
% MN    & 72.12 & 56.81 & 38.31 & 10.46   \\
MN$^\dag$    & 72.08 & 57.61 & 38.34 & 10.34   \\
% MONet & 54.47 & 30.66 & 36.66 & 19.78   \\
MONet$^\dag$ & 61.36 & 45.61 & 35.64 & 23.59   \\
% SA    & 95.89 & 36.61 & 62.40 & 22.58   \\
SA$^\dag$    & 94.88 & 37.68 & 61.60 & 21.96   \\
% IODINE & 93.81 & 45.14 & 59.52 & 29.17   \\
IODINE$^\dag$ & 93.68 & 44.20 & 60.63 & 29.40   \\
% DTI-S & 59.54 & 48.74 & 497.90 & 33.79   \\
DTI-S$^\dag$ & 89.86 & 53.38 & 79.86 & 32.20   \\
% GNM   & 65.05 & 59.92 & 53.37 & 42.25   \\
GNM$^\dag$   & 65.67 & 63.38 & 53.38 & 44.30   \\
% SAVi  & -    & -  & 49.54 & 31.88   \\
% PMP   & 91.69 & 66.70 & 90.80 & 55.07   \\
PPMP$^\dag$   & \underline{95.94} & \underline{84.86} & \underline{92.61} & \textbf{77.67}   \\
% Ours  & 95.03 & 63.36 & 94.66 & 64.08   \\
Ours$^\dag$  & \textbf{96.95} & \textbf{86.38} & \textbf{95.32} & \underline{70.28}    \\ \bottomrule    
\end{tabular}
\caption{\textbf{Multi-Object Segmentation results.} The results here \\are with post-processing. }
\label{tab:clevr-pp}
\end{table}

==> tab/depth_kitti.tex <==
\begin{table*}[b]
\centering
\begin{tabular}{@{}lccccccc@{}}
\toprule
 & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RSME $\downarrow$ & RMSE log $\downarrow$ & $\delta < 1.25$ $\uparrow$ & $ \delta < 1.25^2$ $\uparrow$ & $ \delta < 1.25^3$ $\uparrow$ \\ \midrule
Zhou \etal ~\cite{Zhou2017CVPR} & 0.176 & 1.532& 6.129 & 0.244 & 0.758 & 0.921 & 0.971 \\
Mahjourian \etal ~\cite{Mahjourian2018CVPR} & 0.134 & 0.983& 5.501 & 0.203 & 0.827 & 0.944 & 0.981 \\
GeoNet~\cite{Yin2018CVPR} & 0.132 & 0.994& 5.240 & 0.193 & 0.833 & 0.953 & 0.985 \\
DDVO~\cite{Wang2018CVPR} & 0.126 & 0.866& 4.932 & 0.185 & 0.851 & 0.958 & 0.986 \\
Ranjan \etal ~\cite{Ranjan2019CVPR} & 0.123 & 0.881& 4.834 & 0.181 & 0.860 & 0.959 & 0.985 \\
EPC++~\cite{Luo2019PAMI} & 0.120 & 0.789& 4.755 & 0.177 & 0.856 & 0.961 & 0.987 \\
% Ours & 0.107 & 1.273& 3.976 & 0.150 & 0.912 & 0.976 & 0.989 \\
Ours & 0.107 & 1.539& 4.027 & 0.149 & 0.911 & 0.971 & 0.989 \\
Monodepth2~\cite{Godard2019ICCV} & 0.090 & 0.545& 3.942 & 0.137 & 0.914 & 0.983 & 0.998 \\
PackNet-SfM~\cite{Guizilini2020CVPR} & 0.078 & 0.420& 3.485 & 0.121 & 0.934 & 0.986 & 0.996 \\
\bottomrule
\end{tabular}
\caption{\textbf{Evaluation of Depth Estimation on KITTI.} We use the Eigen split of KITTI using improved ground truth.}
\label{tab:depth-kitti}
\end{table*}

==> tab/old_depth_movi.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
\centering
\begin{tabular}{@{}lcccclccc@{}}
\toprule
Dataset & Abs Rel $\downarrow$ & Sq Rel $\downarrow$ & RSME $\downarrow$ & RMSE log $\downarrow$ & log10 $\downarrow$ & $\delta < 1.25$ $\uparrow$  & $ \delta < 1.25^2$ $\uparrow$ & $ \delta < 1.25^3$ $\uparrow$  \\ \midrule
MOVi-A & 0.113 & 0.348 & 1.483 & 0.226 & 0.061  & 0.813 & 0.912 & 0.949 \\
MOVi-C & 0.225 & 0.604 & 1.845 & 0.299 & 0.100  & 0.609& 0.856 & 0.946 \\
MOVi-D & 0.544 & 2.863 & 3.744 & 1.381 & 0.415 & 0.348 & 0.547 & 0.657 \\
MOVi-E & 0.274 & 1.198 & 2.965 & 0.582 & 0.162 & 0.565 & 0.747 & 0.829 \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth Evaluation on Foreground Objects on MOVi Datasets}.}
\label{tab:old-depth-movi}
\end{table*}

==> tab/seg_kitti.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[b]
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
    & \multicolumn{1}{c}{KITTI}      \\\cmidrule(l){2-2}
Model    & \textbf{FG-ARI} $\uparrow$ \\ \midrule
SA~\cite{Locatello2020NeurIPS} & 13.8 \\
MONet~\cite{Burgess2019ARXIV} & 14.9 \\
SCALOR~\cite{Jiang2020ICLR} & 21.1 \\
S-IODINE~\cite{Greff2019ICML} & 14.4 \\
MCG~\cite{Arbelaez2014CVPR}  & 40.9 \\
Ours & 42.3 \\
Bao \etal ~\cite{Bao2022CVPR} & 47.1 \\
PPMP~\cite{Karazija2022NeurIPS} & 50.8 \\
%PPMP (Swin)~\cite{Karazija2022NeurIPS} & 58.3 \\
% \midrule
% OCLR (test. adap.)     & 64.4 & 65.2  & 63.6 \\
% Ours (test. adap.)     & 62.8 & 63.8  & 61.8 \\
\bottomrule
\end{tabular}
\caption{\textbf{Segmentation Results on KITTI}.}
\label{tab:seg-kitti}
\end{table}
